Understanding the Limitations of Network Online Learning

Studies of networked phenomena, such as interactions in online social media, often rely on incomplete data, either because these phenomena are partially observed, or because the data is too large or expensive to acquire all at once. Analysis of incomplete data leads to skewed or misleading results. In this paper, we investigate limitations of learning to complete partially observed networks via node querying. Concretely, we study the following problem: given (i) a partially observed network, (ii) the ability to query nodes for their connections (e.g., by accessing an API), and (iii) a budget on the number of such queries, sequentially learn which nodes to query in order to maximally increase observability. We call this querying process Network Online Learning and present a family of algorithms called NOL*. These algorithms learn to choose which partially observed node to query next based on a parameterized model that is trained online through a process of exploration and exploitation. Extensive experiments on both synthetic and real world networks show that (i) it is possible to sequentially learn to choose which nodes are best to query in a network and (ii) some macroscopic properties of networks, such as the degree distribution and modular structure, impact the potential for learning and the optimal amount of random exploration.

==> NOL_algorithm.tex <==
\begin{algorithm}
\caption{Network on-line learning (\modname\ ) with random restart}
\begin{algorithmic}[1]
\REQUIRE $\hG_0 \textrm{ (initial incomplete network)}$, $b$ (probing budget),  $\epsilon$ (jump rate), and $\alpha\textrm{ (step-size for gradient descent)}$
\ENSURE $\theta_b \textrm{ (parameters of the learning model)}, \hG_b$ (network after $b$ probes)
	\STATE Initialize: $\theta_0$ (randomly or heuristically); $P_0 = \emptyset$
	\REPEAT 
		\STATE  \textrm{Calculate feature vectors:} $\phi_t(i)$, $ \forall \textrm{ node } i \in \hV_t-P_t$ 
		\STATE  \textrm{Calculate estimated rewards:} $\V_{\theta_t}(i) =\theta_{t}^\textrm{T}\phi_t(i)$ 
		\STATE \textrm{Explore: With probability} $\epsilon$, choose node $u_t \in \hG_0-P_t$ uniformly at random.
		\STATE \textrm{Exploit: With probability} $1-\epsilon$, $u_t = argmax_{i} \left(\theta_{t}^\textrm{T}\phi_t(i)\right)\textrm {,}$ $\,\, \textrm {where } i \in \hV_t-P_t$
		\STATE Probe node $u_t$
		\STATE Update the observed graph: $\hG_{t+1} = \{\hG_t \cup \textrm{ neighbors of }u_t\}$ 
		\STATE Collect reward: $r_t(u_t)= |\hG_{t+1}| - |\hG_t|$
		\STATE Online $loss_t(u_t)=  \left( r_t(u_t) - \V_{\theta_t}(u_t)\right)^2$
		\STATE \textrm{Compute on-line gradient: } \\  $\nabla_{\theta_t}loss_t(u_t) = -2 \left(r_t(u_t) - \V_{\theta_t}(u_t) \right)  \phi_t(u_t)$ 
		\STATE Update parameters: $\theta_{t+1}= \theta_t + \alpha  \nabla_{\theta_t}loss_t(u_t)$
		\STATE $t \leftarrow t+1$
	\UNTIL {t==b}
	\RETURN $\theta_b$ and $\hG_b$ 
\end{algorithmic}
\label{alg:nol}
\end{algorithm}

==> lfr-figure.tex <==
\begin{figure}[ht]
%% mu 0.1/0.2
\begin{subfigure}{0.245\textwidth}
    \includegraphics[width=\linewidth]{figures/LFR-1-new-nodes.pdf}
    \caption{}
    \label{fig:lfr-01}
\end{subfigure}%
\begin{subfigure}{0.245\textwidth}
\includegraphics[width=\linewidth]{figures/LFR-2-new-nodes.pdf}
    \caption{}
    \label{fig:lfr02}
\end{subfigure}
% mu 0.3/0.4
\begin{subfigure}{0.245\textwidth}
    \includegraphics[width=\linewidth]{figures/LFR-3-new-nodes.pdf}
    \caption{}
    \label{fig:lfr-03}
\end{subfigure}%
\begin{subfigure}{0.245\textwidth}
\includegraphics[width=\linewidth]{figures/LFR-4-new-nodes.pdf}
    \caption{}
    \label{fig:lfr04}
\end{subfigure}
    \captionsetup{width=0.9\textwidth}
    \caption{\HTR\ outperforms baseline methods on graphs generated by the LFR community benchmark model \cite{LFR}. The difference in performance is more significant when the mixing parameter $\mu$ is lower, corresponding to higher modularity $Q$, and \HTR\ is able to perform on par with all baselines regardless of $\mu$. \HTR\ also exhibits performance that is considerably more stable than that of NOL. In these results, we fix the degree distribution exponent of the LFR model to $\gamma = 3 $ and the community size distribution exponent $\beta = 2$.}
    \label{fig:LFR}
\end{figure}
